Relational Database Augmented Large Language Model

Large language models (LLMs) excel in many natural language processing (NLP) tasks. However, since LLMs can only incorporate new knowledge through training or supervised fine-tuning processes, they are unsuitable for applications that demand precise, up-to-date, and private information not available in the training corpora. This precise, up-to-date, and private information is typically stored in relational databases. Thus, a promising solution is to augment LLMs with the inclusion of relational databases as external memory. This can ensure the timeliness, correctness, and consistency of data, and assist LLMs in performing complex arithmetic operations beyond their inherent capabilities. However, bridging the gap between LLMs and relational databases is challenging. It requires the awareness of databases and data values stored in databases to select correct databases and issue correct SQL queries. Besides, it is necessary for the external memory to be independent of the LLM to meet the needs of real-world applications. We introduce a novel LLM-agnostic memory architecture comprising a database selection memory, a data value memory, and relational databases. And we design an elegant pipeline to retrieve information from it. Besides, we carefully design the prompts to instruct the LLM to maximize the framework's potential. To evaluate our method, we compose a new dataset with various types of questions. Experimental results show that our framework enables LLMs to effectively answer database-related questions, which is beyond their direct ability.

==> sections/methodology.tex <==
\section{Methodology}

\subsection{Problem Definition}

Our method aims to retrieve necessary information from a collection of relational databases to help LLM in producing accurate and database-specific outputs. In the conventional LM paradigm, both input and output consist of text. However, a common use case of relational databases involves users inputting natural language questions to retrieve specific data from the database systems. So in this work, given the user input, which may or may not require information from relational databases, the expected output could be either a textual string or a result in the form of SQL query outcome.

\subsection{LLM-based Agent}

Retrieving information from a collection of databases to augment LLM is a complicated task that involves multiple steps. So we decompose it into multiple modules and build an autonomous agent to call each module by utilizing the in-context learning ability of LLM. An overview of our method is shown in Figure \ref{fig:overview}.

\subsubsection{Context Switch Module}
Given an input, the agent first determines if a retrieval is needed. A retrieval is redundant if the input already provides enough context to generate output. Determining if a question is answerable based on the context is a classic task for LM~\cite{rajpurkar2018know}. Previous studies have shown that LLMs could address the task with reasonable accuracy~\cite{kocon2023chatgpt}. So we propose to use LLMs to act as the context switch module by letting it decide if the output can be directly extracted from the input context. An example of how the context switch works is shown in Figure \ref{fig:context_switch}.

\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figure/context_switch_prompt.pdf}
    \caption{An example showing the input and output of the context switch module 
    %\YS{keep the same direction for Fig. 1 and Fig. 2}
    \vspace{-3mm}
    }
    \label{fig:context_switch}
\end{figure}

\subsubsection{Database Selection and Planning Module} 

\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figure/planning_prompt.pdf}
    \caption{An example showing the input and output of the database selection and planning module}
    \label{fig:planning_prompt}
\end{figure}

The next step is to select any databases that might contain relevant information. Then the agent generate a retrieval plan for each selected database. Although it is reasonable to divide the database selection and retrieval plan generation into two separate steps, we found that merging them together yields better results in practice. It is because if the agent is only instructed to select relevant databases, it would select false positive databases that are slightly relevant to the input. For example, given a question ``\textit{how many countries have more than three car manufacturers?}'', the agent might select all the databases that contain a table named ``\textit{countries}''.
So, in our database selection and planning module, given a list of candidate databases, the agent is instructed to select databases and generate a retrieval plan in one step, which reduces the selection of false-positive databases. An example of this module is shown in Figure \ref{fig:planning_prompt}

To determine which databases are relevant to the input, the module requires a list of descriptions for the candidate databases as input. Following the paradigm in previous text-to-SQL studies~\cite{pourreza2023din,li2023resdsql}, we use a database schema that consists of the database name, table names, column names, and foreign key relationships. An example of database schema is shown in Figure \ref{fig:schema}. We can see that the database schema provides a brief summarization of what data is stored in the database, which makes it possible to use language models to predict which databases are relevant to the input and what information can be retrieved from it.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figure/schema.pdf}
    \caption{An example of database schema}
    \label{fig:schema}
    \vspace{-3mm}
\end{figure}


To fully exploit the advantages of structured knowledge in relational databases, a retrieval plan should rely on SQL queries to conduct retrieval and analysis of information. But restricted by the SQL syntax, a SQL query can only access one database. So we instruct the LLM to generate retrieval plans consist of multiple sub-goals where each sub-goal describes a retrieval step that can be parsed into a SQL query. Specifically, the module exploits Chain-of-Thought prompting~\cite{wei2022chain} to generate a retrieval plan. 
To ensure each sub-goal can be parsed into a SQL query, the LLM is instructed to generate an example SQL code for each sub-goal. 
%To avoid redundant SQL queries, the module encourages the LLM to generate a minimum number of sub-goals.

The retrieval plan also describes how the results of each sub-goal can contribute to the final output. Notably, in our design the agent relies on the SQL query to conduct retrieval and reasoning of data from one database and relies on the in-context learning ability of LLM to conduct reasoning of data from different databases. Since SQL has a powerful expressiveness that supports a variety of arithmetic, logical, and string operations, the agent is able to perform complicated reasoning over data from one database, which is difficult for knowledge stored in raw text or other unstructured forms. But the cross-database reasoning power of our agent would be limited by the capability of LLMs. However, we believe it is sufficient to handle many real-world applications. 
%Besides, there are many ongoing studies to improve the reasoning ability of LLM by utilizing external tools or more complicate promptings.

Different from previous studies in LLM-based dynamic planning~\cite{yao2022react,shinn2023reflexion}, our retrieval plan is not generated in an auto-regressive way (i.e., generating the next step based on the outcome of the current step). It is because if there are multiple steps accessing different databases, they are likely to be independent of each other. And if a retrieval plan has multiple steps retrieving information from the same database, they can usually be replaced by a nested SQL query, which is more efficient to execute than multiple SQL queries. To encourage the agent to generate nested SQL queries, the LLM is instructed to generate a minimum number of sub-goals.


\subsubsection{Text-to-SQL and Retrieval Module}

\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figure/text_to_sql_prompt.pdf}
    \vspace{-3mm}
    \caption{An example showing the input and output of the text-to-SQL and retrieval module.}
    \label{fig:text2sql}
    \vspace{-3mm}
\end{figure}

Given a database and a sub-goal, the text-to-SQL and retrieval module parses the sub-goal into a SQL query and executes the SQL query to retrieve the results. An example of the module is shown in Figure \ref{fig:text2sql}. Previous studies have shown that LLMs can parse natural language questions into SQL queries with state-of-the-art accuracy. So we follow the latest LLM-based text-to-SQL framework, DIN-SQL~\cite{pourreza2023din}, for text-to-SQL parsing. After SQL is generated, the agent executes it in the corresponding database. Then the SQL query and SQL result are returned as the context for output generation.

To further improve the robustness of text-to-SQL parsing, we propose an extra self-correction step after a SQL query is executed. Differing from the self-correction step in previous text-to-SQL studies~\cite{pourreza2023din}, our self-correction step only applies to inexecutable SQL queries and is based on the error message returned by the database system. Specifically, when receiving the error message, the agent would try to modify the SQL query based on the error message and the database schema. If a SQL query is still inexecutable after several correction attempts, the agent would exclude the query in the output generation process.   


\subsubsection{Output Generation Module.}
After retrieving information from the databases, the last step is to generate outputs based on the user inputs and the retrieved SQL results. Since the output could be either SQL results or text strings, the output generation module needs to determine if one of the SQL results can be directly returned as outputs. To that end, the agent first checks if there is one of the SQL query semantically equivalent to the user input. If there is, then the SQL result of that sub-question is directly returned as output. Otherwise, the module would return text results. To generate the text output, following the approach in~\cite{ram2023context}, we add the SQL and the SQL results into the input context. If a SQL result is too long to be included in the prompt, it is truncated and only the first 10 rows are kept. Since it is possible that some SQL results are actually irrelevant, the LLM is instructed to first identify which SQL is useful and then generate output to the user input. An example of this module is illustrated in Figure \ref{fig:output}. 

\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figure/output_prompt.pdf}
    \caption{An example showing the input and output of the output generation module.}
    \label{fig:output}
    \vspace{-6mm}
\end{figure}

\subsection{Enhancing Agent with Auxiliary Models}

There are two major challenges in the current agent that cannot be resolved by prompt-based in-context learning: database selection scalability and database-value-unawareness during text-to-SQL. In this section, we will discuss the two limitations and introduce the auxiliary models used to address them.

\subsubsection{Enhancing Database Selection Scalability} The first challenge is the scalability of the database selection. Recall that in the database selection and planning module, the input prompt contains the schemas of all candidate databases. Since the prompt length is usually bounded, it is infeasible if the number of databases is large.
To address the issue, we propose to fine-tune a smaller auxiliary language model (LM) as a pruner to predict the probability that the database contains useful information based on its schema and user input. During database selection, the agent sequentially computes the relevance score of each database by calling the model. Only the top-K databases are included in the LLM input prompts for further selection and planning. Figure \ref{fig:database_selection} shows the pipeline of database selection and planning module with the auxiliary database pruner.
%Notably, fine-tuning allows the model to learn a unified criterion to quantify the relevancte between databases and inputs, which is difficult for in-context learning.

Given an user input $\bm{x}$ and a database
$D$, the database pruning can be viewed as a binary classification task. The input would be the concatenation of user input and database schema and the output is a probability score $p_{\bm{x},D}$ between 0 and 1. So the model can be trained with binary cross-entropy loss.
\begin{equation}
    -y_{\bm{x},D}\log p_{\bm{x},D} - (1-y_{\bm{x},D})\log(1-p_{\bm{x},D})
\end{equation}
We augment the training data of two text-to-SQL datasets, Spider~\cite{yu2018spider} and Dr Spider \cite{chang2023dr}, to train the database pruner. In the original datasets, each natural language question is associated with one ground-truth database, which is used as the positive samples in the binary classification task. Negative samples are generated by replacing the ground-truth database with a random one. In addition, to mimic cases where a question requires accessing multiple databases, we concatenate $K$ random questions together as a composite question. A database is considered relevant to a composite question only if it is the ground-truth database for at least one question in the composite question. 

\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figure/database_selection.pdf}
    \caption{An example showing the pipeline of database selection and planning module with the database pruner.}
    \label{fig:database_selection}
\end{figure}

\subsubsection{Database-Value-Aware Text-to-SQL %\YS{make the caption more positive. as in the above caption.}
%\YS{even more positive? Such as Retrieve Values from Database. BTW, check the quotes: ``correct quotes'', "incorrect"}
} 
The second challenge is how to address the errors caused by the unawareness of database values during the text-to-SQL process. 
%\YS{change the wording into: chanllenges and what do we want to achieve.} 
For example, assume there is a table of restaurants where the city Los Angeles is stored as ``LA''. Given a question ``\textit{show me the restaurant located in Los Angeles}'', the correct SQL should be ``
\textit{SELECT name FROM restaurant WHERE location=‘LA’}
''. But if a text-to-SQL model is unaware of the values stored in the table, it is likely to generate ``
\textit{SELECT name FROM restaurant WHERE location=‘Los Angeles’}
'' instead, which is reasonable but would not retrieve any information. A common solution is to fine-tune the text-to-SQL model on the specific database. But in practice, new databases might be added to aid the LLM and the cost to fine-tune a LLM is expensive, so fine-tuning might not be a suitable solution. Another solution is to input all the values in the selected column to the text-to-SQL model, but it is infeasible when the table contains thousands of rows. 

Therefore, we propose to build a semantic retriever to select candidate values from the database. Specifically, given a sub-goal, the text-to-SQL module first parses it into a SQL query by using the values in the questions. Then, a SQL parser identifies the columns and values that appeared in the conditions of the SQL query (e.g., 
[restaurant.location, ‘Los Angeles’] in the previous example
). Next, the retriever searches the cells of the identified columns (location) to find possible value synonyms of the identified value (``LA'') based on their semantic embeddings. Finally, the LLM is prompted to correct the SQL query based on the values retrieved from the database.

To facilitate the search, for each column, an index is built to store the semantic embeddings of all the cells. Given a query value (e.g., ``Los Angeles''), its semantic embedding is computed and used as the query vector of the nearest neighbor search to find the top-K cells with the most similar semantics. The retrieved cells would be the candidate values for SQL. Figure \ref{fig:value-retriever} shows how the value retriever works with our text-to-SQL and retrieval module.

To obtain the semantic embedding of a cell or a query value, a pre-trained language model is used to compute the semantic embeddings of its tokens:
\begin{equation}
    F([t_1,t_2,\cdots,t_n])=[\bm{h}_1,\bm{h}_2,\cdots,\bm{h}_n]
\end{equation}
where $\bm{h}_i$ is the last hidden embedding of token $t_i$ output by the pre-trained LM. Notice that the pre-trained language model does not need fine-tuning because the last-hidden-embeddings of a pre-trained language model could already capture the similarity in token semantics effectively. Then, since the number of tokens in each cell or token value is usually small, its semantic embedding is computed as the average of the token embeddings in it, i.e., 
$\text{Mean}\{\bm{h}_1,\bm{h}_2,\cdots,\bm{h}_n\}$.

\begin{figure}
    \centering
    \includegraphics[width=0.92\linewidth]{figure/value-retriever.pdf}
    \caption{An example showing the pipeline of text-to-SQL and retrieval module with the auxiliary value retrieval model.}
    \label{fig:value-retriever}
    \vspace{-3mm}
\end{figure}
